Behavioral Indicators of Overreliance During Interaction with Conversational Language Models

LLMs are now embedded in a wide range of everyday scenarios. However, their inherent hallucinations risk hiding misinformation in fluent responses, raising concerns about overreliance on AI. Detecting overreliance is challenging, as it often arises in complex, dynamic contexts and cannot be easily captured by post-hoc task outcomes. In this work, we aim to investigate how users' behavioral patterns correlate with overreliance. We collected interaction logs from 77 participants working with an LLM injected plausible misinformation across three real-world tasks and we assessed overreliance by whether participants detected and corrected these errors. By semantically encoding and clustering segments of user interactions, we identified five behavioral patterns linked to overreliance: users with low overreliance show careful task comprehension and fine-grained navigation; users with high overreliance show frequent copy-paste, skipping initial comprehension, repeated LLM references, coarse locating, and accepting misinformation despite hesitation. We discuss design implications for mitigation.

==> 06_findings_qualititive.tex <==

\section{Interview}
\label{sec:qualitative_findings}

\xac{to be cut and merged into discussion}

To further understand users' thought process underlying their interaction behaviors and its connection to overreliance, we conducted an interview with 12 randomly-selected participants following the conclusion of the data collection session.
% Twelve users were randomly selected from the 77 participants to join the interview.
Table \xx presents the 12 participants' detailed overreliance scores (M = \xx, SD = \xx ).
% 
During the data collection part, these participants were instructed to record their interactions using screen-capture software. \xac{only these 12 users did the screen recording? reviewers might question whether this will affect their behavior than other non-recorded participants.}
% The selection process ensured a diverse sample representative of the target population. 
% We analyzed these participants' behavior sequences and their underlying intentions. 
% and demographic information.
% 
% Participants were instructed to record their interactions using screen-capture software. 
The interviewer closely observed the entire interaction process and conducted a 20-minute semi-structured interview after task completion,
% was conducted to gain further understanding of participants' behavior and thought process in relation to overreliance. 
which we reported as follows.
% The interview was conducted in a controlled, in-person setting. 

\xac{how did you analyze the interview data?}

% \xac{did you first analyze their overreliance and then their interaction behaviors?}

% \xac{what's the method of analysis that conclude participants had these following behavior?}
\clcomment{qinyi: we first let users report the process of the whole task, then we find out the point where they are influenced by AI and ask them about the thinking process behind it.}


% \xac{should this be a stand-alone section?}
% Subsequent analysis of the interview data revealed qualitative themes that can align with quantitative findings.

\subsection{Persuasion by AI Through Multi-rounds Interaction with AI} \label{subsubsec:convienced}
First, we observed that users with high overreliance scores tend to be persuaded by the AI’s reasons, especially in multi-rounds interactions. For example, in task 1, P2 expressed an initial disagreement with the AI’s suggestion:
\begin{quote}
    \textit{“There were conflicts... like I thought the compass and map should be together, so I asked why they weren’t. After the AI explained that one item was more important, I ended up adopting its suggestion.”}
\end{quote}

Similarly, P5 noted,
\begin{quote}
    \textit{“I think it had an arrangement that I didn’t agree with at first... but it kind of convinced me to some degree, even though I didn’t fully agree, but it changed my mind... It suggested prioritizing a book over water, arguing that the book could help find water in the desert. I thought, maybe it makes sense.”}
\end{quote}

Other participants showed similar shifts in opinion after arguing with AI. For instance, P1 initially felt a gun was unnecessary but reconsidered after asking the AI about potential wild animal threats:\textit{ “It said they were present, so I moved the gun up in priority.”} P6, who questioned why oxygen should be prioritized over a communicator, noted, \textit{“The AI explained that carrying too much weight could hinder movement in space. It seemed logical, so I followed its suggested order.” }
% \xac{reflect on literature on using XAI to prevent overreliance}


For the lower-reliant participants, they exhibit a self-calibration mechanism for task offloading. When they detect an AI error, they turn to independent thinking rather than arguing with the AI or seeking explanations.

% \colorbox{lightgray}{
\textbf{Connection to patterns of interaction behaviors}:
Echoing the potential findings in Section \ref{subsubsec:deliberating_vs_wavering}, where we propose that users become more overreliant on the \ai as they are more wavering, we claim that this increased reliance may stem from users gradually being persuaded by the AI during multi-turn conversations. \xac{need rewriting.}



% Besides, we also find some behavior patterns that  ..... have not been detected by aligned with quantitative findings:

\subsection{Awareness Variation in AI-Output Evaluation}
% 需要区分ai literacy

Quantitative results reveal two distinct metacognitive profiles \xac{cite the metacognition paper} among low-overreilance \xac{low-overreilance?} and high-overreilance, differentiated by their ability to articulate AI’s limitations:

\textbf{High-awareness users with Explicit Deficit Recognition}:
Low-reliant users explicitly identify AI’s contextual mismatches thus can adapt outputs strategically when making revision. For example, P2 noted, \textit{“In the end, I found that some of the AI-generated tips were overly general, so I made further adjustments.”} Also, P7 mentioned, \textit{“I read the summary generated, and there are some places where details were missing. So I went in and added pieces to correct it.”}

\textbf{Low-awareness users with Intuitive Detection}:
In contrast, \hol like P1 exhibit experiential and intuitive monitoring, revising based on perceptual discomfort (\textit{"noticed new things needing tweaking"}) without articulating specific AI errors. This reflects lower-order metacognition---detecting output-ideal mismatches through iterative comparison rather than explicit flaw identification.

\textbf{Connection to patterns of interaction behaviors}:
The Low-awareness users can also tend to revise with uncertainty and make more wavering in the process, potentially exacerbating overreliance as mentioned in Section \ref{subsubsec:deliberating_vs_wavering}. \xac{the connection is weak. need rewriting}


\subsection{Problem Decomposition with Targeted AI Queries \xac{this heading needs rewriting}}
\label{subsec:problem_decomposition}
Low-reliance users exhibit a pattern of problematizing tasks into decontextualized queries, consulting the AI only on fragmented aspects without sharing full task context. For example, P4 in the survival task asked \textit{"How does a signal mirror function in extreme cold?"} without disclosing the broader scenario, indicating self-guided task decomposition. These queries often appear tangential, but reflect users' strategic cognitive offloading to verify specific hypotheses.

This contrasts with \hol won't decompose tasks, as \lol retain control over problem framing and solution integration. Their interactions demonstrate selective AI dependency, leveraging the tool to validate micro-decisions while maintaining macro-task autonomy.

Users should be well aware of the the types of information in the task that the \ai is likely to make mistakes on (such as time and price) and will actively double-check such information via search engine. This conclusion echoes with previous research \cite{jacobs2021machine}.

\textbf{Connection to patterns of interaction behaviors}: \xac{???}


\subsection{Workflow Adaptation for Error Mitigation}
\xac{moved this from discussion to here}
Low-reliance users exhibit proactive workflow modification by inserting external validation steps into their task execution.
For example, P7 identified AI's price inaccuracies and turned to search engine for verification. This behavior reflects metacognitive awareness of AI's limitations, specifically its susceptibility to outdated or contextually mismatched information.
Low-reliant users retain greater autonomy in choosing between AI-generated contents and external sources. For example, P8 shared, \textit{“At first, I asked GPT for some general suggestions, reviewed its response briefly, and then went online to find more updated travel guides.”}

However, while consulting external sources offers greater accuracy, it can also increase the time required to complete a task, a trade-off we will further discuss in Section \ref{subsec:discussion_time}

\textbf{Connection to patterns of interaction behaviors}: \xac{???}
